OmniActions: Predicting Digital Actions in Response to Real-World Multimodal Sensory Inputs with LLMs

The progression to "Pervasive Augmented Reality" envisions easy access to multimodal information continuously. However, in many everyday scenarios, users are occupied physically, cognitively or socially. This may increase the friction to act upon the multimodal information that users encounter in the world. To reduce such friction, future interactive interfaces should intelligently provide quick access to digital actions based on users' context. To explore the range of possible digital actions, we conducted a diary study that required participants to capture and share the media that they intended to perform actions on (e.g., images or audio), along with their desired actions and other contextual information. Using this data, we generated a holistic design space of digital follow-up actions that could be performed in response to different types of multimodal sensory inputs. We then designed OmniActions, a pipeline powered by large language models (LLMs) that processes multimodal sensory inputs and predicts follow-up actions on the target information grounded in the derived design space. Using the empirical data collected in the diary study, we performed quantitative evaluations on three variations of LLM techniques (intent classification, in-context learning and finetuning) and identified the most effective technique for our task. Additionally, as an instantiation of the pipeline, we developed an interactive prototype and reported preliminary user feedback about how people perceive and react to the action predictions and its errors.

==> content/06_02_f1scores.tex <==

\subsubsection{F1 Scores When Predicting Follow-Up Actions}
To further analyze the role of the imbalanced data, we used F1 scores to evaluate whether the techniques could achieve better performance when performing top-3 predictions.

For a label $L$, \textit{recall} measures how well a model identifies all relevant instances, while \textit{precision} measures the model's accuracy in its positive predictions. The F1 score is the harmonic mean of these two measures. As precision and recall are often competing metrics, F1 scores should provide a more balanced understanding of the model's performance.
% Our data shows that the actions people intend to take on multimodal information are not evenly distributed (Figure \ref{fig:action_dist}).
% For example, 
Thus, we individually calculated precision and recall for each label, then aggregated these metrics by weighting them to calculate the overall weighted F1-scores across all labels. The precision and recall for a label $L$ was calculated as:
\begin{equation}
\begin{split}
    \text{Precision}_{L} &= \frac{TP_{L}}{TP_{L} + FP_{L}} \\
    \text{Recall}_{L} &= \frac{TP_{L}}{TP_{L} + FN_{L}}
\end{split}
\end{equation}

where
\begin{itemize}
    \item \textbf{True positives ($TP_{L}$)}: the count of instances where label $L$ was correctly predicted and is in the ground truth.
    \item \textbf{False positives ($FP_{L}$))}: the count of instances where label $L$ was missed as a ground truth label and when $L$ is predicted but not in the ground truth. This is, for a single data entry, \(FP_{L} = \frac{1+\text{Number of other incorrect labels}}{\text{Number of missed ground truth labels}}\)
    \item \textbf{False negatives ($FN_{L}$)}: the count of instances were label $L$ is in the ground truth but not predicted.
\end{itemize}


By using the number appearances of each label as the weights, we calculated the weighted F1 scores of the model as:
\begin{equation}
    \text{F1}_{W} = \frac{2 \times \text{Precision}_{W} \times \text{Recall}_{W}}{\text{Precision}_{W} + \text{Recall}_{W}}
\end{equation}

The results showed that while merely predicting the dominant actions can achieve high recall, it results in low precision (Table \ref{tab:accuracy_comparison_f1}  and Appendix \xx). It perform poorly when the number of labels increased (i.e., predicting specific actions).
% Analyzing these numbers yields several insights:
% \begin{itemize}
%     \item While merely predicting the dominant actions can achieve high recall, it results in low precision. It perform poorly when the number of labels increases (i.e., predicting specific actions).
%     \item While in-context learning approach have zero knowledge of the distribution of the collected data, it outperformed other approaches, showing that a large model trained on massive world information may be able to generalize to new tasks when providing proper instructions.
%     \item While 
% \end{itemize}

\input{tables/comparison_f1.tex}


==> tables/comparison_f1.tex <==
\begin{table}[ht]
    \centering
    \color{blue}
    \caption{F1-score (\%) when predicting top-3 actions of different approaches.
    % \nick{separating the prediction on two different modalities} 
    }
    
    \renewcommand{\arraystretch}{1.1} % reduce the row height
    \begin{tabular}{C{4.1cm}*{6}{C{1.2cm}}}
    
    
      & \multicolumn{3}{c}{\textbf{Predicting General}} & \multicolumn{3}{c}{\textbf{Predicting Specific}} \\
     \hline
    \centering{Approach} & Recall  & Precision & F1-score & Recall  & Precision & F1-score  \\ 
    \hline
        
    \hline
    
    \textit{Predicting 3 most-dominant only}          &     \textbf{0.862}     &     0.744       &   0.799  &  0.542  &  0.324 &  0.406 \\ 
    Intent classification (davinci)          &      0.737          &     0.746   &  0.741 &  0.521 & 0.453 & 0.485 \\ 
    Fine-tuning (GPT-3.5)          &  0.743        &       0.705    & 0.714 &  0.520  &  0.479  &  0.499     \\
    In-context learning (GPT-3.5)         &      0.758        &     0.746  & 0.752 &  0.410  &  0.477 &  0.441  \\ 
    In-context learning (GPT-4)         & 0.838             &     \textbf{0.837}  & \textbf{0.837} &  \textbf{0.633} &  \textbf{0.657}  &  \textbf{0.645}  \\
    \bottomrule
    \end{tabular}
    \label{tab:accuracy_comparison_f1}
\end{table}

==> tables/diary_examples_table.tex <==
% \begin{tabularx}{\textwidth}{c|X|X|X|X|X|X|X|X|X|X|}

% % \# & \centering 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
% % \hline
% Type 1 & & & & & & & & & & \\
% \hline
% Row 2 & & & & & & & & & & \\
% \hline
% Row 3 & & & & & & & & & & \\
% \hline
% Row 4 & & & & & & & & & & \\
% \hline
% Row 5 & & & & & & & & & & \\
% \hline
% \end{tabularx}

% \begin{tabularx}{\textwidth}{|c|*{10}{>{\centering\arraybackslash}X|}}

% % \# &  1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
% \hline
% Type & \faImage & \faHeadphones & Photo & Photo & Photo & Photo & \faVideo & Video & Photo & Photo \\
% \hline
% Action & & & & & & & & & & \\
% \hline
% % Row 3 & & & & & & & & & & \\
% % \hline
% % Row 4 & & & & & & & & & & \\
% % \hline
% % Row 5 & & & & & & & & & & \\
% % \hline
% \end{tabularx}

% \begin{tabularx}{\textwidth}{|c|c|X|c|}

% \hline
% \# & Type & \centering Action & Category \\
% \hline
% 1 & \faImage &  & [MERGE] \\
% \hline
% 2 & \faHeadphones &  & [MERGE] \\
% \hline

% \end{tabularx}

% \begin{tabularx}{\textwidth}{|c|c|X|c|}

% \hline
% \# & Type & \centering Action & Category \\
% \hline
% 1 & \faImage & Share this fun moment on Instagram & \multirow{2}{*}{Share}  \\
% \cline{1-3}
% 2 & \faHeadphones & Send it to a garage maintenance person to diagnose the problem &  \\
% \hline
% 3 & \faImage & Take a photo of it to keep record of my son's painting progress & \multirow{2}{*}{Save}  \\
% \cline{1-3}
% 4 & \faImage & Save this receipt so I could send it for reimbursement after the trip &  \\
% \hline
% 5 & \faImage & Search the keyboard on google lens to buy one for me & \multirow{2}{*}{Query}  \\
% \cline{1-3}
% 6 & \faImage & Search online to know what are “APPLE FRITTERS.” &  \\
% \hline
% 7 & \faHeadphones & Transcribe the professor’s lecture and save as note for later to review & \multirow{4}{*}{Others}  \\
% \cline{1-3}
% 8 & \faVideo & Zoom in to see the seal more clearly &  \\
% \cline{1-3}
% 9 & \faImage & Translate some of the dishes to my native language &   \\
% \cline{1-3}
% 10 & \faImage & Set a reminder for next week for when the homework is due &  \\
% \hline

% \end{tabularx}


\begin{tabularx}{\textwidth}{|c|c|X|}
\hline
\textbf{\#} & \textbf{Type} & \textbf{Action} \\
\hline
1 & \faImage & Share this fun moment on Instagram. \\
\cline{1-3}
2 & \faHeadphones & Send it to a garage maintenance person to diagnose the problem. \\
\hline
3 & \faImage & Keep record of my son's painting progress. \\
\cline{1-3}
4 & \faImage & Save this receipt and send for reimbursement later. \\
\hline
5 & \faImage & Search the keyboard on google lens to buy one. \\
\cline{1-3}
6 & \faImage & Search “APPLE FRITTERS” online. \\
\hline
7 & \faHeadphones & Transcribe the professor’s lecture. \newline Save as note for later to review. \\
\cline{1-3}
8 & \faVideo & Zoom in to see the seal more clearly. \\
\cline{1-3}
9 & \faImage & Translate some of the dishes to my native language. \\
\cline{1-3}
10 & \faImage & Set a reminder for next week's homework due. \\
\hline

\multicolumn{3}{p{0.9\textwidth}}{\footnotesize \textit{\#2 is an abnormal clicking sound of a garage door opening.}
\newline
\textit{\#7 is an audio of professor talking about the history of the United States.}
}
\end{tabularx}

% \multicolumn{3}{>{\hsize=\dimexpr2\hsize+3\tabcolsep+\arrayrulewidth\relax}X}{\footnotesize \#2 is an abnormal clicking sound of a garage door opening. \newline
% \#7 is a professor talking about the history of the United States.
% }
% \multicolumn{3}{l}{\footnotesize Note: \#2 is an abnormal clicking sound of a garage door opening.} \\
% \multicolumn{3}{l}{\footnotesize \# 7 is a professor talking about the history of the United States.}

% {\footnotesize Note: \#2 is an abnormal clicking sound of a garage door opening.  \newline
% \#7 is a professor talking about the history of the United States.}
% \begin{tabularx}{\textwidth}{|c|c|X|}
% \hline
% \textbf{\#} & \textbf{Type} & \textbf{Action} \\
% \hline
% 1 & \faImage & Share this fun moment on Instagram. \\
% \cline{1-3}
% 2 & \faHeadphones & Send it to a garage maintenance person to diagnose the problem. \\
% \hline
% 3 & \faImage & Keep record of my son's painting progress. \\
% \cline{1-3}
% 4 & \faImage & Save this receipt and send for reimbursement later. \\
% \hline
% 5 & \faImage & Search the keyboard on google lens to buy one. \\
% \cline{1-3}
% 6 & \faImage & Search “APPLE FRITTERS” online. \\
% \hline
% 7 & \faHeadphones & Transcribe the professor’s lecture. \newline Save as note for later to review. \\
% \cline{1-3}
% 8 & \faVideo & Zoom in to see the seal more clearly. \\
% \cline{1-3}
% 9 & \faImage & Translate some of the dishes to my native language. \\
% \cline{1-3}
% 10 & \faImage & Set a reminder for next week's homework due. \\
% \hline
% \multicolumn{3}{p{\linewidth}}{\footnotesize \#2 is an abnormal clicking sound of a garage door opening.
% \newline
% \#7 is a professor talking about the history of the United States.
% } \\

